Cost Efficient High Capacity Indoor Wireless Access: Denser Wi-Fi or Coordinated Pico-cellular?

Rapidly increasing traffic demand has forced indoor operators to deploy more and more Wi-Fi access points (APs). As AP density increases, inter-AP interference rises and may limit the capacity. Alternatively, cellular technologies using centralized interference coordination can provide the same capacity with the fewer number of APs at the price of more expensive equipment and installation cost. It is still not obvious at what demand level more sophisticated coordination pays off in terms of total system cost. To make this comparison, we assess the required AP density of three candidate systems for a given average demand: a Wi-Fi network, a conventional pico-cellular network with frequency planning, and an advanced system employing multi-cell joint processing. Numerical results show that dense Wi-Fi is the cheapest solution at a relatively low demand level. However, the AP density grows quickly at a critical demand level regardless of propagation conditions. Beyond this Wi-Fi network limit, the conventional pico-cellular network works and is cheaper than the joint processing in obstructed environments, e.g., furnished offices with walls. In line of sight condition such as stadiums, the joint processing becomes the most viable solution. The drawback is that extremely accurate channel state information at transmitters is needed.

==> intro_old <==
\section{Introduction}
% increasing demand and popular WLAN for indoor deployment
Wireless data traffic rapidly increases over last few years triggered by mobile handset innovation, e.g., tablet PCs or smartphones. Operators have aggressively deployed IEEE 802.11 based WLANs for offloading to mitigate the explosive traffic burden to existing outdoor networks.
Main driver behind the WLAN popularity is that it thus far provided significantly low deployment cost compared to other cellular solutions, e.g., picocells or distributed antenna systems~\cite{VJ08TMCOM}.
As the trend of data traffic growth is foreseen to continue and is even accelerated by bandwidth-hungry applications, e.g., real-time cloud computing or web-storage service, operators are tempted to deploy more and more WLANs.

\subsection{Motivations and Related Work}
Increasing WLAN density creates more interference with more frequent media access contention among co-channel access points~(APs) for downlink transmission.
With the lack of centralized coordination, such inter-AP interference may result in a negative impact on overall network capacity. Nevertheless, there were not so many studies which explored a large scale of WLAN deployment owing to its complex behavior of distributed coordinated function~(DCF)~\cite{Nguyen2007,Alfano2011,Johansson2007vtc,Simic2012}.  For instance, authors in~\cite{Nguyen2007,Alfano2011} proposed analytical methods based on stochastic geometry and evaluated the spatial average over random AP locations. They presumed infinite deployment areas and homogeneous channel gain statistics for analytical tractability. Instead, other studies executed more flexible simulation based studies under average inter-AP interference, underestimating the network performance~\cite{Johansson2007vtc,Simic2012}.

A conventional cellular network more sophisticatedly deals with interference at relatively more expensive equipment and installation cost whereas a dense WLAN network relies only on CSMA/CA for inter-AP interference coordination. It statically allocates a different sub-band in each AP\footnote{Without the loss of generality, we use a term AP for a transmitter in a cellular network at the rest of paper instead of using a commonly used base station.} in a centralized manner, but it adaptively determines a frequency reuse number according to propagation conditions, so-called frequency planning.
% JP
As one evolutionary path in the cellular track, multi-cell joint processing techniques often named as networked MIMO, e.g., linear coordinated beamforming, have been demonstrated as another promising mean to combat interference (see~\cite{Gesbert2010} and references therein for the survey of recent results on the various multi-cell joint processing).
%
This comes at the expenses of installing costly optical fibers for fast information exchange between APs.
% related work in a cellular
Separated from WLAN literature, most works in a cellular domain have showed the superiority of the various joint processing schemes for the fixed number of APs~\cite{Karakayali2006,Jing2008,Boudreau2009,Gesbert2010}.
%A recent paper provided a comprehensive survey on multi-cell joint processing techniques~\cite{Gesbert2010}.
%
Relatively few numbers of studies compared the densification of two cellular approaches in a classical hexagonal cellular array~\cite{Liang2008,Marsch2010}.


%While actual cost figure varies on market situations, the number of deployed APs can be an alternative indicator for financial comparison of candidate systems since the AP density is almost linear to the total network cost~\cite{JS97VTC}.
%Moreover, due to the wide variety of in-building structures that leads to different interference characteristics~\cite{}, the tightly coordinated system may lose its performance advantage in some environments.
%Typical WLAN network analysis often assumed all APs and users in carrier sensing range and measured collisions (outage in a cellular context) without exploiting the gain of rate adaptation, e.g. see~\cite{Bianchi2000}, for analysis convenience.

% financial comparison ignoring ICIC difference
% comparing considering ICIC difference is itself rare
%
While tighter interference coordination certainly provides higher network performance, it is not so straightforward if it has financial benefit for future towering indoor user demand.
In techno-economic literature, several financial comparisons between WLAN and cellular solutions usually base on a simple arithmetic capacity estimation with exact empirical cost figures~\cite{phdthesis07johansson,Jan10iofc,Markendahl2011}. However, they disregard the distinct interference coordination mechanisms in each wireless system.
Contrarily, the majority of technical studies on WLAN and cellular systems have thus far overlooked the importance of analyzing the economic benefit of one system than the others when yielding the same network capacity.
Moreover, they often ignored obstructed indoor environments that may weaken the total cost benefit of a system employing more advanced coordination.


\subsection{Contributions and Organization}
The objective of our study is providing an insight into the potential way forward the future low-cost indoor deployments, based on the comparative studies of system options from both WLAN and cellular tracks.
%
In this paper, we explicitly aim to address the following questions:
\begin{itemize}
\item Can WLAN densification provide the cost saving compared with other centrally coordinated cellular solutions for a high capacity indoor deployment?
\item If not, which can be an alternative cellular solution, a conventional cellular network or the multi-cell joint processing and where?
\end{itemize}
While exact cost figures are market and vendor specific, assessing the required AP density to meet a given expected user demand can be seen as a step toward financial advantage evaluation because total network cost is approximately linear to it~\cite{JS97VTC}.
In this regard, we compare the AP density of three wireless systems for a given average user demand: a WLAN network, a conventional cellular network with frequency planning, and multi-cell zero-forcing (ZF) beamforming.
We now detail the main contributions of this work by means of the following list:
\begin{enumerate}
\item First, we quantitatively assess the required AP density of three distinguished systems yielding the same network capacity under the given propagation condition, taking into account technical difference in the interference coordination.
\item Secondly, the AP density of each system is quantified and compared according to increasing average user demand level.
\item Thirdly, we develop an upper bound performance evaluation method of a dense WLAN network which explicitly model the important CSMA/CA operations.
\item Fourthly, the impacts of indoor wall loss and pathloss exponents on the AP density comparison are examined.
\item Lastly, we provide an intuitive economical wireless solution map depending average user demand and propagation conditions based on the quantitative results.
\end{enumerate}
The paper is organized as follows. Section II provides overall system model including network dimensioning and traffic assumptions. Then, a WLAN and cellular network model are given in Section III and IV, respectively. Section V describes a simulation methodology to estimate an individual system performance. Numerical results illustrate implications on the economic future indoor deployment in Section VI. Finally, we draw conclusions in Section VII.
% 0) corroborate with a simplified model and support existing result in individual system
% 0-1) With the best knowledge, none of existing performance evaluation methodologies cannot capture non-homogeneous environments.
% 1) quantitative performance comparison with the considered metric & constraints
% 2) for this, common performance metric with realistic constraint: # of required BSs comparison with respect to a given average aggregate data rates per outage constraint
% 3) comparison according to local environmental difference



% CSI error considerations for

%Due to the wide variety of in-building structures that leads to different interference characteristics~\cite{Rappaport2002}, the impact of WLAN densification should be carefully investigated as well.
%In general, a large-scale WLAN deployment is mathematically very hard to accurately analyze or extremely time-consuming in packet-level simulation due to its complex behavior of distributed coordinated function~(DCF).
%Such system performance benefits, however, often ignored inherent and fundamental errors in channel state information at transmitters (CSIT), when the fading channel is varying in time and frequency.
%the researches on cellular interference management in a cellular network were very broad.
% rare work on comparison densification vs. JP

%, potentially leading high investment to meet the required user demand.
%
%Therefore, a crucial question is which solution can yield the lowest total network cost among both WLAN and the cellular candidates for the up-rising future user demand.
%Obviously, the advanced cellular network requires fewer number of APs than WLANs at the expense of more cost per AP.
%
%In general, the number of placed APs is approximately linear to the total network cost, we can implicitly
%Therefore, the required deployment density, comparison to yield  the same capacity is essential toward the economic investigation.
%
%%
%Accordingly, comparing quantitatively the required density of existing a WLAN network and a cellular network is an essential step and identifying the feasibility of the joint processing in more realistic environments and propagation conditions.
%
%There are also two distinct approaches in a cellular domain to deal with interference with extra cost in equipments: centralized frequency division in picocells and smart distributed antenna with joint multicell processing~\cite{VJ08TMCOM}.
%%
%%

% related work
% 1) financial comparison~\cite{} with empirical cost figures without considering inter-AP interference in dense WLAN networks
% 2) direct financial comparison with more sophisticated modeled interference coordination is essential due to fundamental difference in interference coordination.
% 3) while realistic cost figures are varying in market and total network cost is almost linear to the number of deployed APs~\cite{}, quantitative comparison on required number of APs will be a basis for economic investigation of different system solutions


% rare dense WLAN evaluation due to its simulation and analytical complexity
%The complex behavior in the high density of APs is still far to be fully understood when incorporating a realistic description at the physical layer.
%{Bicket2005}.
% no attempts to direct comparison in the same environment and demand conditions



